End-to-End Video Text Spotting with Transformer

Recent video text spotting methods usually require the three-staged pipeline, i.e., detecting text in individual images, recognizing localized text, tracking text streams with post-processing to generate final results. These methods typically follow the tracking-by-match paradigm and develop sophisticated pipelines. In this paper, rooted in Transformer sequence modeling, we propose a simple, but effective end-to-end video text DEtection, Tracking, and Recognition framework (TransDETR). TransDETR mainly includes two advantages: 1) Different from the explicit match paradigm in the adjacent frame, TransDETR tracks and recognizes each text implicitly by the different query termed text query over long-range temporal sequence (more than 7 frames). 2) TransDETR is the first end-to-end trainable video text spotting framework, which simultaneously addresses the three sub-tasks (e.g., text detection, tracking, recognition). Extensive experiments in four video text datasets (i.e.,ICDAR2013 Video, ICDAR2015 Video, Minetto, and YouTube Video Text) are conducted to demonstrate that TransDETR achieves state-of-the-art performance with up to around 8.0% improvements on video text spotting tasks. The code of TransDETR can be found at https://github.com/weijiawu/TransDETR.

==> table/table3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{l|ccc}
% \whline
\scriptsize 
\multirow{2}{*}{Method} & \multicolumn{3}{c}{Video Text Tracking/\%} \\
\cline{2-4} 
& ${\rm ID_{F1}}$$\uparrow$  & ${\rm MOTA}$$\uparrow$ & ${\rm MOTP}$$\uparrow$ \\
\whline
Zuo \textit{et al.}~\cite{zuo2015multi} & - & 56.4 & 73.1 \\
Geometry descriptor~\cite{yu2021end} & - & 74.0 & 76.7  \\
AGD\&AGD~\cite{yu2021end} & - & 75.6 & 74.7  \\
AGD\&EAGD~\cite{yu2021end} & - & 81.3 & 75.7  \\
\rowcolor{mygray}
\detr(ours) & 76.6 & 86.5\green{(+5.2)} & 75.5  \\

% \whline
\end{tabular}

==> table/table5.tex <==

\begin{tabular}{l|ccc}
% \whline
\scriptsize 
Method & Precision  & Recall & F-measure \\
\whline
ours,w/o AOBM & 73.7 & 65.1 & 68.5 \\
ours,w/ AOBM($L1$) & 83.4 & 82.5 & 82.9  \\
ours,w/ AOBM($Cosine$) & 86.2 & \textbf{82.4} & \textbf{84.3}\green{(+15.8)}  \\

% \whline
\end{tabular}



==> table/table6.tex <==

\begin{tabular}{l|ccc}
% \whline
\scriptsize 
Method & ${\rm ID_{F1}}$$\uparrow$  & ${\rm MOTA}$$\uparrow$ & ${\rm MOTP}$$\uparrow$ \\
\whline
ours,w/o AOBM & 73.7 & 65.1 & 68.5 \\
ours,w/ AOBM($L1$) & 83.4 & 82.5 & 82.9  \\
ours,w/ AOBM($Cosine$) & 86.2 & \textbf{82.4} & \textbf{84.3}\green{(+15.8)}  \\

% \whline
\end{tabular}



==> table/table7.tex <==

\begin{tabular}{l|ccccc}
% \whline
\scriptsize 
Length & ${\rm ID_{F1}}$$\uparrow$  & ${\rm MOTA}$$\uparrow$ & ${\rm MOTP}$$\uparrow$ & ${\rm M\mbox{-}Tracked}$$\uparrow$ & ${\rm M\mbox{-}Lost}$$\downarrow$ \\
\whline
% 2 & 59.2 & 42.1 & 76.2 & 36.7 & 30.2 \\
3 & 61.2 & 44.8 & 76.1 & 38.9 & 32.6 \\
4 & 63.4 & 45.5 & 75.9 & 40.1 & 33.2 \\
5 & 65.2 & 47.1 & 75.9 & 42.0 & 31.5 \\
6 & 65.5 & 47.5 & 76.2 & 43.4 & 31.3 \\

% \whline
\end{tabular}



==> table/table9.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{l|cccc|cccc}
% \whline
\scriptsize 

$\tau_{en}$ & 0.4  & 0.5 & 0.6 & 0.7 & 0.4  & 0.5 & 0.6 & 0.7 \\
$\tau_{ex}$ & 0.3  & 0.4 & 0.5 & 0.6 & 0.2  & 0.3 & 0.4 & 0.5 \\
\hline
${\rm ID_{F1}}$$\uparrow$ & 67.5  & 67.5 & 66.6 & 63.3 & 66.6  & \textbf{67.7} & 66.8 & 63.5 \\
${\rm MOTA}$$\uparrow$ & 53.8  & \textbf{54.4} & 53.3 & 48.3  & 53.5 & 54.3 & 53.8 & 48.8\\
${\rm MOTP}$$\uparrow$ & 76.8  & 77.0 &  77.4 & \textbf{77.8}  & 76.7 & 76.9 & 77.3 & \textbf{77.8}\\


% \whline
\end{tabular}



==> table/table_all.tex <==
\begin{subtable}
	\centering
	\setlength{\tabcolsep}{1.2mm}
	\small 
	\begin{tabular}{l|ccc}
    % \whline
    Method & Precision  & Recall & F-measure \\
    \hline
    ours,w/o AOBM & 67.7 & 56.1 & 61.5 \\
    ours,w/ AOBM($L1$) & 77.4 & \textbf{70.5} & 73.8  \\
    ours,w/ AOBM($Cosine$) & \textbf{80.6} & 70.2 & \textbf{75.0}  \\
    
    % \whline
    \end{tabular}
    \caption{Arbitrary-Oriented Box Matching(AOBM) for text detection task on ICDAR2015~(video frames)~\cite{karatzas2015icdar}}
	\label{table:icdar15}
	\vspace{2mm}
\end{subtable}
\quad
\begin{subtable}
	\centering
	\setlength{\tabcolsep}{1.2mm}
	\small 
	\begin{tabular}{l|ccc}
    % \whline
    Method & ${\rm ID_{F1}}$$\uparrow$  & ${\rm MOTA}$$\uparrow$ & ${\rm MOTP}$$\uparrow$ \\
    \hline
    ours,w/o AOBM & 41.1 & 18.4 & 68.7 \\
    ours,w/ AOBM($L1$) & 63.3 & 45.6 & 76.1  \\
    ours,w/ AOBM($Cosine$) & \textbf{65.5} & \textbf{47.5} & \textbf{76.2}  \\
    
    % \whline
    \end{tabular}
    \caption{Arbitrary-Oriented Box Matching(AOBM) for text tracking task on ICDAR2015~(video)~\cite{karatzas2015icdar}.}
	\label{table:icdar15video}
	\vspace{2mm}
\end{subtable}
\quad
\begin{subtable}
	\centering
	\setlength{\tabcolsep}{0.9mm}
	\small
	\begin{tabular}{l|ccccc}
    Length & ${\rm ID_{F1}}$$\uparrow$  & ${\rm MOTA}$$\uparrow$ & ${\rm MOTP}$$\uparrow$ & ${\rm M\mbox{-}Tracked}$$\uparrow$ & ${\rm M\mbox{-}Lost}$$\downarrow$ \\
    \hline
    % 2 & 59.2 & 42.1 & 76.2 & 36.7 & 30.2 \\
    3 & 61.2 & 44.8 & 76.1 & 38.9 & 32.6 \\
    4 & 63.4 & 45.5 & 75.9 & 40.1 & 33.2 \\
    5 & 65.2 & 47.1 & 75.9 & 42.0 & 31.5 \\
    6 & \textbf{65.5} & \textbf{47.5} & \textbf{76.2} & \textbf{43.4} & \textbf{31.3} \\
    
    % \whline
    \end{tabular}
    \caption{The input video frame length for text tracking task on ICDAR2015~(video)~\cite{karatzas2015icdar}.}
	\label{table:length}
	\vspace{2mm}
\end{subtable}
\quad
\begin{subtable}
    \small
	\centering
	\setlength{\tabcolsep}{1.2mm}
	\small
	\begin{tabular}{l|ccccc}
    Layers & GFLOPS/FPS & \#params & ${\rm ID_{F1}}$  & ${\rm MOTA}$ & ${\rm MOTP}$  \\
    \hline
    3 & 94/10.4 & 38M & 61.6 & 44.6 & 76.3 \\
    4 & 104/9.8 & 39M & 64.3 & 46.4 & 76.6 \\
    5 & 114/8.9 & 40M & 65.1 & 47.2 & 76.3 \\
    6 & 124/8.4 & 41M & \textbf{65.5} & \textbf{47.5} & \textbf{76.2} \\
    
    \end{tabular}
    \caption{Effect of encoder size for text tracking task on ICDAR2015~(video)~\cite{karatzas2015icdar}.}
	\label{table:encoder}
	\vspace{2mm}
\end{subtable}

==> table/table_all_2.tex <==
\scriptsize 
\begin{tabular}{l|ccc}
    % \whline
    Method & ${\rm ID_{F1}}$$\uparrow$  & ${\rm MOTA}$$\uparrow$ & ${\rm MOTP}$$\uparrow$ \\
    \hline
    ours,w/o AOBM & 41.1 & 18.4 & 68.7 \\
    ours,w/ AOBM($L1$) & 63.3 & 45.6 & 76.1  \\
    ours,w/ AOBM($Cosine$) & \textbf{65.5} & \textbf{47.5} & \textbf{76.2}  \\
    
    % \whline
\end{tabular}

==> table/table_all_4.tex <==
% \scriptsize 
\begin{tabular}{l|ccccc}
    Layers & GFLOPS/FPS & \#params & ${\rm ID_{F1}}$  & ${\rm MOTA}$ & ${\rm MOTP}$  \\
    \hline
    % 2 & 59.2 & 42.1 & 76.2 & 36.7 & 30.2 \\
    3 & 94/10.4 & 38M & 61.6 & 44.6 & 76.3 \\
    4 & 104/9.8 & 39M & 64.3 & 46.4 & 76.6 \\
    5 & 114/8.9 & 40M & 65.1 & 47.2 & 76.3 \\
    6 & 124/8.4 & 41M & \textbf{65.5} & \textbf{47.5} & \textbf{76.2} \\
    
    
    % \whline
    \end{tabular}

==> table/tables.tex <==
\begin{subtable}[t]{3.2in}
	\centering
	\setlength{\tabcolsep}{1.2mm}
	\small 
	\begin{tabular}{l|ccc}
    % \whline
    Method & Precision  & Recall & F-measure \\
    \hline
    ours,w/o MOBM & 67.7 & 56.1 & 61.5 \\
    ours,w/ MOBM($L1$) & 77.4 & \textbf{70.5} & 73.8  \\
    ours,w/ MOBM($Cosine$) & \textbf{80.6} & 70.2 & \textbf{75.0}  \\
    
    % \whline
    \end{tabular}
    \caption{Multi-Oriented Box Matching(MOBM) for text detection task on ICDAR2015~(video frames)~\cite{karatzas2015icdar}}
	\label{table:icdar15}
	\vspace{2mm}
\end{subtable}
\quad
\begin{subtable}[t]{3.2in}
	\centering
	\setlength{\tabcolsep}{1.2mm}
	\small 
	\begin{tabular}{l|ccc}
    % \whline
    Method & ${\rm ID_{F1}}$$\uparrow$  & ${\rm MOTA}$$\uparrow$ & ${\rm MOTP}$$\uparrow$ \\
    \hline
    ours,w/o MOBM & 41.1 & 18.4 & 68.7 \\
    ours,w/ MOBM($L1$) & 63.3 & 45.6 & 76.1  \\
    ours,w/ MOBM($Cosine$) & \textbf{65.5} & \textbf{49.5} & \textbf{74.1}  \\
    
    % \whline
    \end{tabular}
    \caption{Multi-Oriented Box Matching(MOBM) for text tracking task on ICDAR2015~(video)~\cite{karatzas2015icdar}.}
	\label{table:icdar15video}
	\vspace{2mm}
\end{subtable}
\quad
\begin{subtable}[t]{3.2in}
	\centering
	\setlength{\tabcolsep}{0.9mm}
	\small
	\begin{tabular}{l|ccccc}
    Length & ${\rm ID_{F1}}$$\uparrow$  & ${\rm MOTA}$$\uparrow$ & ${\rm MOTP}$$\uparrow$ & ${\rm M\mbox{-}Tracked}$$\uparrow$ & ${\rm M\mbox{-}Lost}$$\downarrow$ \\
    \hline
    % 2 & 59.2 & 42.1 & 76.2 & 36.7 & 30.2 \\
    3 & 61.2 & 44.8 & 74.0 & 35.1 & 37.6 \\
    5 & 63.4 & 45.5 & 74.0 & 35.4 & 35.1 \\
    7 & 65.2 & 47.8 & \textbf{74.3} & 36.1 & 34.3 \\
    9 & \textbf{65.5} & \textbf{49.5} & 74.1 & \textbf{37.2} & \textbf{33.3} \\
    
    % \whline
    \end{tabular}
    \caption{The input video frame length for text tracking task on ICDAR2015~(video)~\cite{karatzas2015icdar}.}
	\label{table:length}
	\vspace{2mm}
\end{subtable}
\quad
\begin{subtable}[t]{3.2in}
    \small
	\centering
	\setlength{\tabcolsep}{1.2mm}
	\small
% 	\begin{tabular}{l|ccccc}
%     Layers & GFLOPS/FPS & \#params & ${\rm ID_{F1}}$  & ${\rm MOTA}$ & ${\rm MOTP}$  \\
%     \hline
%     3 & 94/10.4 & 38M & 61.6 & 49.6 & 74.0 \\
%     4 & 104/9.8 & 39M & 64.3 & 48.4 & 74.0 \\
%     5 & 114/8.9 & 40M & 65.0 & 49.2 & 74.2 \\
%     6 & 124/8.4 & 41M & \textbf{65.5} & \textbf{49.5} & \textbf{74.1} \\
    
    \begin{tabular}{l|ccc}
    % \whline
    \scriptsize 
    Method & ${\rm ID_{F1}}$$\uparrow$  & ${\rm MOTA}$$\uparrow$ & ${\rm MOTP}$$\uparrow$ \\
    % \whline
    \hline
    IoU-based & 56.3 & 43.1 & 75.8 \\
    Transcription-based & 56.9 & 43.5 & 75.9  \\
    % \rowcolor{mygray}
    Text Query & \textbf{65.5} & \textbf{49.5} & \textbf{74.1}  \\
    
    % \whline
    \end{tabular}
    \caption{Effect of Text Query-based for Text Tracking Task. Deformable-DETR~\cite{zhu2020deformable} is used as the base detector for text tracking on ICDAR2015 (video)~\cite{karatzas2015icdar}. The related settings of IoU and Transcription-based follows the work~\cite{wang2017end}.}
    

	\label{table:encoder}
	\vspace{2mm}
\end{subtable}
